DMT-JEPA: Discriminative Masked Targets for Joint-Embedding Predictive Architecture

The joint-embedding predictive architecture (JEPA) recently has shown impressive results in extracting visual representations from unlabeled imagery under a masking strategy. However, we reveal its disadvantages, notably its insufficient understanding of local semantics. This deficiency originates from masked modeling in the embedding space, resulting in a reduction of discriminative power and can even lead to the neglect of critical local semantics. To bridge this gap, we introduce DMT-JEPA, a novel masked modeling objective rooted in JEPA, specifically designed to generate discriminative latent targets from neighboring information. Our key idea is simple: we consider a set of semantically similar neighboring patches as a target of a masked patch. To be specific, the proposed DMT-JEPA (a) computes feature similarities between each masked patch and its corresponding neighboring patches to select patches having semantically meaningful relations, and (b) employs lightweight cross-attention heads to aggregate features of neighboring patches as the masked targets. Consequently, DMT-JEPA demonstrates strong discriminative power, offering benefits across a diverse spectrum of downstream tasks. Through extensive experiments, we demonstrate our effectiveness across various visual benchmarks, including ImageNet-1K image classification, ADE20K semantic segmentation, and COCO object detection tasks. Code is available at: \url{https://github.com/DMTJEPA/DMTJEPA}.

==> SECTIONS/40_Experiments/exp_vis_seg.tex <==
\begin{figure}[t]
\centering
\fbox{\rule{0pt}{3in}
\rule{0.8\linewidth}{0pt}}
% \includegraphics[width=0.9\linewidth]{figs/vis_seg.pdf}
% \vspace{0.01em}
\caption{Qualtitative visualization of video segmentation results on the DAVIS 2017 benchmark.
\todo{}
}
% \vspace{-0.3cm}
\label{fig: exp_vis_seg}
\end{figure}

